Sim2real gap is non-monotonic with robot complexity for morphology-in-the-loop flapping wing design

Morphology of a robot design is important to its ability to achieve a stated goal and therefore applying machine learning approaches that incorporate morphology in the design space can provide scope for significant advantage. Our study is set in a domain known to be reliant on morphology: flapping wing flight. We developed a parameterised morphology design space that draws features from biological exemplars and apply automated design to produce a set of high performance robot morphologies in simulation. By performing sim2real transfer on a selection, for the first time we measure the shape of the reality gap for variations in design complexity. We found for the flapping wing that the reality gap changes non-monotonically with complexity, suggesting that certain morphology details narrow the gap more than others, and that such details could be identified and further optimised in a future end-to-end automated morphology design process.

==> 6_thanks.tex <==
\section{Acknowledgments}

Acknowledgments omitted for anonymous review
%The authors would like to thank the support of [W]the Defence Science and Technology Group and the Trusted Autonomy Systems Strategic Research Initiative.
